Public Sphere 2.0: Targeted Commenting in Online News Media

With the increase in online news consumption, to maximize advertisement revenue, news media websites try to attract and retain their readers on their sites. One of the most effective tools for reader engagement is commenting, where news readers post their views as comments against the news articles. Traditionally, it has been assumed that the comments are mostly made against the full article. In this work, we show that present commenting landscape is far from this assumption. Because the readers lack the time to go over an entire article, most of the comments are relevant to only particular sections of an article. In this paper, we build a system which can automatically classify comments against relevant sections of an article. To implement that, we develop a deep neural network based mechanism to find comments relevant to any section and a paragraph wise commenting interface to showcase them. We believe that such a data driven commenting system can help news websites to further increase reader engagement.

==> analysis.tex <==
\section{Analysis}
Given the annotated paragraph-comment pairs, we carry out some statistical analysis to get a preliminary insight of the comment structure. At the very outset, we observe the distribution of relevance scores for the paragrpah-comment pairs for different articles for both the Guardian ant NYT dataset.
As evident from Figure \ref{fig:Score_dist}, a majority of comment-paragraph pairs are irrelevant. However, it is imperative to state that this distribution of low score does not necessarily translate that a comment is irrelevant throughout. There are certain comments which are pertinent to specific paragraphs as opposed to the entire article. 

Figure \ref{fig:rel-spike} demonstrates the importance of a comment centered around one paragraph, while the figures, Figure \ref{fig:avg-score}, \ref{fig:low-score}, \ref{fig:high-score} highlights a comment which is of moderate, low and high relevance respectively throughout the entire article.
Although such examples are shown from the Guardian dataset, the same trend holds for the NYT news articles as well. 


\todo{Ritam's work}
We have also noted the average relevance of a comment across the article length. Simply put, we wanted to observe whether relevant comments occur at specific paragraphs of an article or are they distributed randomly throughout its length. 
The article \cite{nielsen2003usability} has noted that users predominately read online Web pages in an F-shaped pattern i.e two horizontal stripes followed by a vertical stripe, clearly seen in \ref{fig:f-heatmap}.  
This implies that attention span of users wanes as they read an article and most of their attention is focused on the initial paragraphs. This behavior is strongly pronounced in our observation that the mean relevance of a comment decreases along the article's length as seen in Figure \ref{fig:mean_para_rel}. This exemplifies that more relevant comments are related to the beginning paragraphs of an article and such a trend holds true for both Guardian and NYT articles. The slight peak at the end of an article's length reflects the concluding content of a news article and is often a reiteration of the beginning paragraphs. 


\begin{figure}[h]
   	\centering
   	\includegraphics[width=.5\textwidth]{Figures/Score_dist.png} 
   	\caption{Frequency of relevant  comments}
   	~\label{fig:Score_dist}   
 
\end{figure} 

\begin{figure}[h]   	
	\centering
	\begin{subfigure}[b]{0.21\textwidth}
		\includegraphics[width=\textwidth]{Figures/peak.png}
		\caption{Specific relevance}
		\label{fig:rel-spike}
	\end{subfigure}
	\begin{subfigure}[b]{0.21\textwidth}
		\includegraphics[width=\textwidth]{Figures/avg.png}
		\caption{Moderate relevance}
		\label{fig:avg-score}
	\end{subfigure}
	\begin{subfigure}[b]{0.21\textwidth}
		\includegraphics[width=\textwidth]{Figures/low.png}
		\caption{Low relevance}
		\label{fig:low-score}
	\end{subfigure}
	\begin{subfigure}[b]{0.21\textwidth}
		\includegraphics[width=\textwidth]{Figures/good.png}
		\caption{High relevance}
		\label{fig:high-score}
	\end{subfigure}
\end{figure}

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}[b]{0.2\textwidth}
% 		\includegraphics[width=\textwidth]{Figures/Fheatmap.png}
% 		\caption{F-shaped heatmap detected by eye-tracking}
% 		\label{fig:f-heatmap}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.2\textwidth}
% 		\includegraphics[width=\textwidth]{Figures/Rel_length.png}
% 		\caption{Mean Comment relevance across an article}
% 		\label{fig:mean_para_rel}
% 	\end{subfigure}
	
% % 	\includegraphics[width=.5\textwidth]{} 
% % 	\caption{Average relevance of each paragraph}
% % 	~\label{fig:mean_para_rel}   
% \end{figure} 

\begin{figure}[h]
   	\centering
   	\includegraphics[width=.5\textwidth]{Figures/Fheatmap.png} 
   \caption{F-shaped heatmap detected by eye-tracking}
	~\label{fig:f-heatmap}
\end{figure} 

 \begin{figure}[h]
   	\centering
   	\includegraphics[width=.45\textwidth, height=7.0cm ]{Figures/Rel_length.png}
		\caption{Mean Comment relevance across an article's length}
		\label{fig:mean_para_rel}
\end{figure} 


==> results.tex <==
\section{Experiments and Results}
\subsection{Experiment Setup}
We apply different Machine Learning classification techniques and finally a deep learning model in order to accomplish the classification task. 

For the machine learning models different feature sets were used. We explored unigram(f1), bigram(f2), trigram(f3)  along with the POS tags(f4) and LIWC(f5) features for both paragraph and the comments. The features considered are appended to form a feature matrix and on it we perform dimensionality reduction using LSA before passing it on to the machine learning classifier. 

For the deep learning model no explicit feature matrix construction using POS or LIWC is required. For this model, we first construct the paragraph and comment vectors as described beforehand in the model description. These are passed on to the model which finally outputs th probability distribution of the class of this paragraph-comment pair . 

\subsection{Training and Testing setup}
For each of the classification models we have used a 10-fold cross validation approach.
Since the number of samples is not that huge, cross validation helps us to test the robustness of our models in the best possible manner rather than using a held out validation and test set. 

For the deep learning model, we have trained for 5 epochs for each step in the 10-fold cross validation.

\subsection{Results}
We have only considered the F-score values for evaluation of our models. The macro, micro and weighted average f-scores for each model for both the datasets are listed below :

% \begin{table*}[!htb]
% \centering
% \caption{My caption}
% \label{my-label}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
%  & \multicolumn{6}{l|}{The Guardian} & \multicolumn{6}{l|}{New York Times} \\ \hline
%  & \multicolumn{3}{l|}{Precision} &\multicolumn{3}{l|}{Recall} & \multicolumn{3}{l|}{Precision} &\multicolumn{3}{l|}{Recall}  \\ \hline
% Model & Macro   & Micro   & Weighted   & Macro   & Micro   & Weighted   & Macro   & Micro   & Weighted   & Macro   & Micro   & Weighted     \\ \hline
% NB & 46.2   & 42.6   & 61.6   & 42.6   & 42.5  & 42.6   &  33.9  & 35.2   & 60.9   & 40.9 & 35.2& 35.2 \\ \hline
% DT &  42.9  & 49.6   & 53.5   & 35.6   & 50.9  & 50.9   & 36.9   & 59.2   &52.7 & 31.2  &59.1& 59.2\\ \hline
% RF & 37.9   & 44.7   & 45.1   & 24.4   & 44.6  & 44.7   & 17.5   & 57.6   & 37.8   &20.2 &57.3& 57.6 \\ \hline
% K-NN &  48.5  & 63.5   & 61.3   & 48.1   & 63.4  & 63.5   & 37.6   & 58.9   & 55.9   & 34.8&61.2&61.2  \\ \hline
% R-SVM &  49.9  & 63.1   & 60.9   & 45.4   & 63.0  & 63.1   &  39.4  & 61.9   & 51.9 &27.3& 61.9 & 60.3  \\ \hline
% AdaBoost &  38.3  & 49.3   & 48.2   & 35.7   & 49.3  & 49.2   & 29.3   & 56.1   & 48.1&28.5& 55.1   &54.6   \\ \hline
% LR &  41.2  & 54.0   & 51.3   & 38.8   & 54.1  & 54.0   & 34.1   & 60.6   & 50.7   &25.8 &60.7&60.1  \\ \hline

% DL-LSTM &  64.1  & 74.4   & 74.5   &  63.6  & 74.5  &  73.3  & 56.6   & 76.8   &76.1 &57.8& 76.9  &76.8   \\ \hline
% DL-GRU &  \textbf{64.2}  & \textbf{75.3}   & \textbf{75.9}   & \textbf{63.7}   & \textbf{75.3}  &  \textbf{75.4}  &  \textbf{64.8}  & \textbf{79.1}   &\textbf{78.4}  &\textbf{64.3}& 7\textbf{79.3} & \textbf{79.1}  \\ \hline
% \end{tabular}
% \end{table*}







\iffalse{}
\subsection{Metrics}
For evaluating the model we have considered F-score metric. Since this is a multi-class classification we have calculated macro, micro and weighted average of the f-scores of each class. The formulas are listed below.

Let $TP_i$, $FP_i$, $TN_i$ and $FN_i$ be the number of true positives, false positives, true negatives and false negatives respectively for each class $i$. Let $P_i$, $R_i$ and $F_i$ denoted the precision, recall and f-score respectively of each class $i$. 
Also let $N$ be total number of classes (here $N = 5$), and $Count_i$ represents the number of samples of each class $i$.
\begin{equation}
P_i = \frac{TP_i}{TP_i + FP_i}
\end{equation}
\begin{equation}
R_i = \frac{TP_i}{TP_i + FN_i}
\end{equation}
\begin{equation}
F_i = \frac{2 \times P_i \times R_i}{P_i + R_i}
\end{equation}

\textbf{Macro Metrics}
\begin{equation}
\textit{Macro Precision} = \frac{\sum_{i=1}^{N} P_i}{N}
\end{equation}
\begin{equation}
\textit{Macro Recall} = \frac{\sum_{i=1}^{N} P_i}{N}
\end{equation}
\begin{equation}
Macro F-score = \frac{2 \times \textit{Macro Precision} \times \textit{Macro Recall}}{\textit{Macro Precision} + \textit{Macro Recall}}
\end{equation}

\textbf{Micro Metrics}
\begin{equation}
\textit{Micro Precision} = \frac{\sum_{i=1}^{N} TP_i}{\sum_{i=1}^{N} (TP_i + FP_i)}
\end{equation}
\begin{equation}
\textit{Micro Recall} = \frac{\sum_{i=1}^{N} TP_i}{\sum_{i=1}^{N} (TP_i + FN_i)}
\end{equation}
\begin{equation}
Micro F-score = \frac{2 \times \textit{Micro Precision} \times \textit{Micro Recall}}{\textit{Micro Precision} + \textit{Micro Recall}}
\end{equation}

\textbf{Weighted Average Metric}
\begin{equation}
\textit{Weighted average F-score} = \frac{\sum_{i=1}^{N} (F_i \times Count_i)}{\sum_{i=1}^{N} Count_i}
\end{equation}
\fi


\iffalse{}
\begin{table}
  \centering
  \caption{F1-Scores for Guardian Dataset}
  \label{table:guardian}
  \scalebox{0.65}{
  \begin{tabular}{|c|c|c|c|c|}
  \hline
  Model & Feature Set & Macro & Micro & Weighted \\
  \hline
  \multirow{12}{4.5em}{Naive Bayes} & f1 & 0.283 & 0.329 & 0.297 \\
   & f2 & 0.305 & 0.353 & 0.344 \\
  & f3 & 0.361 & 0.41 & 0.415 \\
  & f1 + f4 & 0.3 & 0.335 & .315\\
  & f2 + f4 & 0.311 & 0.354 & 0.355\\
  & f3 + f4 & 0.359 & 0.407 & 0.421\\
  & f1 + f5 & 0.305 & 0.343 & 0.327\\
  & f2 + f5 & 0.347 & 0.389 & 0.391\\
  & f3 + f5 & 0.377 & 0.426 & 0.439 \\
  & f1 + f4 + f5 & 0.319 & 0.354 & 0.353\\
  & f2 + f4 + f5 & 0.332 & 0.37 & 0.377\\
  & f3 + f4 + f5 & 0.369 & 0.42 & 0.438\\
  \hline
  \multirow{12}{4.5em}{Decision Tree} & f1 & 0.280 & 0.442 & 0.393 \\
   & f2 & 0.330 & 0.476 & 0.444 \\
   & f3 & 0.295 & 0.477 & 0.413 \\
  & f1 + f4 & 0.319 & 0.491 & 0.447 \\
  & f2 + f4 & 0.349 & 0.492 & 0.467 \\
   & f3 + f4 & 0.339 & 0.48 & 0.456 \\
   & f1 + f5 & 0.291 & 0.477 & 0.409\\
   & f2 + f5 & 0.357 & 0.524 & 0.481  \\
  & f3 + f5 & 0.331 & 0.499 & 0.452 \\
  & f1 + f4 + f5 & 0.345 & 0.509 & 0.473 \\
  & f2 + f4 + f5 & 0.333 & 0.501 & 0.454 \\
   & f3 + f4 + f5 & 0.333 & 0.496 & 0.456 \\

  \hline
  \multirow{12}{4.5em}{Random Forest} & f1 & 0.184 & 0.435 & 0.306 \\
  & f2 & 0.183 & 0.431 & 0.305 \\
  & f3 & 0.219 & 0.453 & 0.339 \\
  & f1 + f4 & 0.171 & 0.429 & 0.293 \\
  & f2 + f4 & 0.202 & 0.445 & 0.324 \\
  & f3 + f4 & 0.201 & 0.444 & 0.321 \\
  & f1 + f5 & 0.18 & 0.436 & 0.303 \\
  & f2 + f5 & 0.195 & 0.444 & 0.317 \\
  & f3 + f5 & 0.206 & 0.446 & 0.327\\
  & f1 + f4 + f5 & 0.168 & 0.43 & 0.29\\
  & f2 + f4 + f5 & 0.187 & 0.445 & 0.31\\
  & f3 + f4 + f5 & 0.199 & 0.447 & 0.321\\
  \hline
  \multirow{12}{4.5em}{Nearest Neighbors} & f1 & 0.423 & 0.577 & 0.554 \\
   & f2 & 0.406 & 0.569 & 0.544 \\
   & f2 & 0.433 & 0.577 & 0.560 \\
   & f1 + f4 & 0.45 & 0.611 & 0.591 \\
   & f2 + f4 & 0.449 & 0.613 & 0.592 \\
   & f3 + f4 & 0.473 & 0.63 & 0.613 \\
   & f1 + f5 & 0.43 & 0.586 & 0.564 \\
   & f2 + f5 & 0.408 & 0.569 & 0.546\\
   & f3 + f5 & 0.446 & 0.597 & 0.579\\
   & f1 + f4 + f5 & 0.457 & 0.616 & 0.596 \\
   & f2 + f4 + f5 & 0.458 & 0.617 & 0.597 \\
   & f3 + f4 + f5 & 0.478 & 0.635 & 0.619 \\
  \hline
  % Linear SVM & f1 & 0.116 & 0.411 & 0.239 \\
  % Linear SVM & f2 & 0.116 & 0.411 & 0.239 \\
  % Linear SVM & f3 & 0.116 & 0.411 & 0.239 \\
  % Linear SVM & f1 + f5 & 0.116 & 0.411 & 0.239 \\
  % Linear SVM & f2 + f5 & 0.116 & 0.411 & 0.239 \\
  % \hline
  \multirow{12}{4.5em}{RBF SVM} & f1 & 0.427 & 0.593 & 0.559 \\
   & f2 & 0.416 & 0.583 & 0.553 \\
   & f3 & 0.441 & 0.607 & 0.580 \\
   & f1 + f4 & 0.431 & 0.603 & 0.567 \\
   & f2 + f4 & 0.45 & 0.62 & 0.591 \\
   & f3 + f4 & 0.467 & 0.636 & 0.608\\
   & f1 + f5 & 0.437 & 0.604 & 0.571\\
   & f2 + f5 & 0.418 & 0.586 & 0.556\\
   & f3 + f5 & 0.449 & 0.613 & 0.586\\
   & f1 + f4 + f5 & 0.436 & 0.607 & 0.571\\
   & f2 + f4 + f5 & 0.447 & 0.618 & 0.587\\
   & f3 + f4 + f5 & 0.461 & 0.63 & 0.599\\
  \hline
  \multirow{12}{4.5em}{Adaboost} & f1 & 0.288 & 0.434 & 0.402 \\
   & f2 & 0.322 & 0.452 & 0.426 \\
   & f3 & 0.310 & 0.454 & 0.426 \\
   & f1 + f4 & 0.322 & 0.45 & 0.429 \\
   & f2 + f4 & 0.316 & 0.452 & 0.427 \\
   & f3 + f4 & 0.344 & 0.481 & 0.458 \\
   & f1 + f5 & 0.345 & 0.476 & 0.454 \\
   & f2 + f5 & 0.332 & 0.463 & 0.439 \\
   & f3 + f5 & 0.342 & 0.477 & 0.456 \\
   & f1 + f4 + f5 & 0.339  & 0.469 & 0.454 \\
   & f2 + f4 + f5 & 0.34  & 0.474 & 0.453 \\
   & f3 + f4 + f5 & 0.357  & 0.493 & 0.475 \\
  \hline
  \multirow{12}{4.5em}{Logistic Regression} & f1 & 0.255 & 0.423 & 0.366 \\
   & f2 & 0.282 & 0.450 & 0.397 \\
   & f3 & 0.328 & 0.484 & 0.441 \\
   & f1 + f4 & 0.319 & 0.468 & 0.434 \\
   & f2 + f4 & 0.339 & 0.487 & 0.455 \\
   & f3 + f4 & 0.37 & 0.519 & 0.491 \\
   & f1 + f5 & 0.285 & 0.455 & 0.403 \\
   & f2 + f5 & 0.302 & 0.471 & 0.421 \\
   & f3 + f5 & 0.35 & 0.504 & 0.467 \\
   & f1 + f4 + f5 & 0.345 & 0.498 & 0.465 \\
   & f2 + f4 + f5 & 0.359 & 0.512 & 0.482 \\
   & f3 + f4 + f5 & 0.39 & 0.54 & 0.514 \\
  \hline
  DL\_LSTM & - & 0.638 & 0.744 & 0.739 \\ 
  \hline
  DL\_GRU & - & 0.634 & 0.753 & 0.748 \\
  \hline
  \end{tabular}
  }
\end{table}

\begin{table}
\centering
\caption{Precision Scores for Guardian Dataset}
\label{table:guardian}
\scalebox{0.65}{
\begin{tabular}{|c|c|c|c|c|}
\hline
Model & Feature Set & Macro & Micro & Weighted \\
\hline
\hline\multirow{12}{4.5em}{Naive Bayes}&f1&0.405&0.329&0.552\\
&f2&0.428&0.353&0.589\\
&f3&0.454&0.41&0.613\\
&f1+f4&0.409&0.335&0.55\\
&f2+f4&0.423&0.354&0.58\\
&f3+f4&0.45&0.407&0.603\\
&f1+f5&0.406&0.343&0.542\\
&f2+f5&0.446&0.389&0.595\\
&f3+f5&0.462&0.426&0.616\\
&f1+f4+f5&0.424&0.354&0.567\\
&f2+f4+f5&0.428&0.37&0.576\\
&f3+f4+f5&0.446&0.42&0.598\\
\hline\multirow{12}{4.5em}{Decision Tree}&f1&0.338&0.442&0.418\\
&f2&0.365&0.476&0.457\\
&f3&0.42&0.477&0.497\\
&f1+f4&0.362&0.491&0.468\\
&f2+f4&0.371&0.492&0.477\\
&f3+f4&0.43&0.48&0.542\\
&f1+f5&0.382&0.477&0.462\\
&f2+f5&0.414&0.524&0.507\\
&f3+f5&0.43&0.499&0.514\\
&f1+f4+f5&0.391&0.509&0.496\\
&f2+f4+f5&0.405&0.501&0.495\\
&f3+f4+f5&0.429&0.496&0.535\\
\hline\multirow{12}{4.5em}{Random Forest}&f1&0.35&0.435&0.422\\
&f2&0.367&0.431&0.439\\
&f3&0.43&0.453&0.497\\
&f1+f4&0.296&0.429&0.372\\
&f2+f4&0.382&0.445&0.456\\
&f3+f4&0.396&0.444&0.464\\
&f1+f5&0.337&0.436&0.412\\
&f2+f5&0.353&0.444&0.427\\
&f3+f5&0.429&0.446&0.496\\
&f1+f4+f5&0.289&0.43&0.366\\
&f2+f4+f5&0.362&0.445&0.433\\
&f3+f4+f5&0.379&0.447&0.45\\
\hline\multirow{12}{4.5em}{Nearest Neighbors}&f1&0.436&0.577&0.549\\
&f2&0.417&0.569&0.538\\
&f3&0.443&0.577&0.554\\
&f1+f4&0.46&0.611&0.585\\
&f2+f4&0.458&0.613&0.585\\
&f3+f4&0.479&0.63&0.605\\
&f1+f5&0.443&0.586&0.558\\
&f2+f5&0.415&0.569&0.537\\
&f3+f5&0.458&0.597&0.577\\
&f1+f4+f5&0.469&0.616&0.591\\
&f2+f4+f5&0.479&0.617&0.59\\
&f3+f4+f5&0.485&0.635&0.613\\
\hline\multirow{12}{4.5em}{RBF SVM}&f1&0.478&0.593&0.579\\
&f2&0.441&0.583&0.554\\
&f3&0.463&0.607&0.58\\
&f1+f4&0.487&0.603&0.591\\
&f2+f4&0.477&0.62&0.593\\
&f3+f4&0.498&0.636&0.612\\
&f1+f5&0.478&0.604&0.583\\
&f2+f5&0.442&0.586&0.556\\
&f3+f5&0.48&0.613&0.591\\
&f1+f4+f5&0.494&0.607&0.596\\
&f2+f4+f5&0.477&0.618&0.59\\
&f3+f4+f5&0.499&0.63&0.609\\
\hline\multirow{12}{4.5em}{AdaBoost}&f1&0.305&0.434&0.398\\
&f2&0.344&0.452&0.425\\
&f3&0.331&0.454&0.426\\
&f1+f4&0.343&0.45&0.424\\
&f2+f4&0.342&0.452&0.434\\
&f3+f4&0.364&0.481&0.458\\
&f1+f5&0.383&0.476&0.461\\
&f2+f5&0.353&0.463&0.44\\
&f3+f5&0.368&0.477&0.462\\
&f1+f4+f5&0.35&0.469&0.453\\
&f2+f4+f5&0.363&0.474&0.454\\
&f3+f4+f5&0.38&0.493&0.482\\
\hline\multirow{12}{4.5em}{Logistic Regression}&f1&0.312&0.423&0.391\\
&f2&0.333&0.45&0.416\\
&f3&0.398&0.484&0.478\\
&f1+f4&0.347&0.468&0.437\\
&f2+f4&0.363&0.487&0.456\\
&f3+f4&0.396&0.519&0.494\\
&f1+f5&0.33&0.455&0.416\\
&f2+f5&0.346&0.471&0.435\\
&f3+f5&0.399&0.504&0.486\\
&f1+f4+f5&0.376&0.498&0.47\\
&f2+f4+f5&0.385&0.512&0.484\\
&f3+f4+f5&0.412&0.54&0.513\\

\hline
  DL\_LSTM & - & 0.638 & 0.744 & 0.739 \\
  \hline
  DL\_GRU & - & 0.634 & 0.753 & 0.748 \\
  \hline
\end{tabular}
}
\end{table}


\begin{table}
  \centering
  \caption{Recall scores for Guardian Dataset}
  \label{table:guardian}
  \scalebox{0.65}{
  \begin{tabular}{|c|c|c|c|c|}
  \hline
  Model & Feature Set & Macro & Micro & Weighted \\
  \hline\multirow{12}{4.5em}{Naive Bayes}&f1&0.35&0.329&0.329\\
&f2&0.372&0.353&0.353\\
&f3&0.42&0.41&0.41\\
&f1+f4&0.37&0.335&0.335\\
&f2+f4&0.372&0.354&0.354\\
&f3+f4&0.406&0.407&0.407\\
&f1+f5&0.366&0.343&0.343\\
&f2+f5&0.402&0.389&0.389\\
&f3+f5&0.422&0.426&0.426\\
&f1+f4+f5&0.379&0.354&0.354\\
&f2+f4+f5&0.386&0.37&0.37\\
&f3+f4+f5&0.402&0.42&0.42\\
\hline\multirow{12}{4.5em}{Decision Tree}&f1&0.298&0.442&0.442\\
&f2&0.331&0.476&0.476\\
&f3&0.303&0.477&0.477\\
&f1+f4&0.339&0.491&0.491\\
&f2+f4&0.361&0.492&0.492\\
&f3+f4&0.36&0.48&0.48\\
&f1+f5&0.302&0.477&0.477\\
&f2+f5&0.356&0.524&0.524\\
&f3+f5&0.334&0.499&0.499\\
&f1+f4+f5&0.355&0.509&0.509\\
&f2+f4+f5&0.337&0.501&0.501\\
&f3+f4+f5&0.356&0.496&0.496\\
\hline\multirow{12}{4.5em}{Random Forest}&f1&0.234&0.435&0.435\\
&f2&0.232&0.431&0.431\\
&f3&0.255&0.453&0.453\\
&f1+f4&0.226&0.429&0.429\\
&f2+f4&0.246&0.445&0.445\\
&f3+f4&0.244&0.444&0.444\\
&f1+f5&0.232&0.436&0.436\\
&f2+f5&0.241&0.444&0.444\\
&f3+f5&0.246&0.446&0.446\\
&f1+f4+f5&0.225&0.43&0.43\\
&f2+f4+f5&0.238&0.445&0.445\\
&f3+f4+f5&0.244&0.447&0.447\\
\hline\multirow{12}{4.5em}{Nearest Neighbors}&f1&0.424&0.577&0.577\\
&f2&0.409&0.569&0.569\\
&f3&0.433&0.577&0.577\\
&f1+f4&0.453&0.611&0.611\\
&f2+f4&0.451&0.613&0.613\\
&f3+f4&0.475&0.63&0.63\\
&f1+f5&0.43&0.586&0.586\\
&f2+f5&0.411&0.569&0.569\\
&f3+f5&0.446&0.597&0.597\\
&f1+f4+f5&0.457&0.616&0.616\\
&f2+f4+f5&0.459&0.617&0.617\\
&f3+f4+f5&0.48&0.635&0.635\\
\hline\multirow{12}{4.5em}{RBF SVM}&f1&0.419&0.593&0.593\\
&f2&0.415&0.583&0.583\\
&f3&0.441&0.607&0.607\\
&f1+f4&0.423&0.603&0.603\\
&f2+f4&0.447&0.62&0.62\\
&f3+f4&0.462&0.636&0.636\\
&f1+f5&0.43&0.604&0.604\\
&f2+f5&0.416&0.586&0.586\\
&f3+f5&0.445&0.613&0.613\\
&f1+f4+f5&0.427&0.607&0.607\\
&f2+f4+f5&0.443&0.618&0.618\\
&f3+f4+f5&0.454&0.63&0.63\\
\hline\multirow{12}{4.5em}{AdaBoost}&f1&0.293&0.434&0.434\\
&f2&0.323&0.452&0.452\\
&f3&0.312&0.454&0.454\\
&f1+f4&0.323&0.45&0.45\\
&f2+f4&0.317&0.452&0.452\\
&f3+f4&0.344&0.481&0.481\\
&f1+f5&0.341&0.476&0.476\\
&f2+f5&0.33&0.463&0.463\\
&f3+f5&0.34&0.477&0.477\\
&f1+f4+f5&0.34&0.469&0.469\\
&f2+f4+f5&0.337&0.474&0.474\\
&f3+f4+f5&0.357&0.493&0.493\\
\hline\multirow{12}{4.5em}{Logistic Regression}&f1&0.264&0.423&0.423\\
&f2&0.29&0.45&0.45\\
&f3&0.324&0.484&0.484\\
&f1+f4&0.32&0.468&0.468\\
&f2+f4&0.339&0.487&0.487\\
&f3+f4&0.368&0.519&0.519\\
&f1+f5&0.291&0.455&0.455\\
&f2+f5&0.309&0.471&0.471\\
&f3+f5&0.346&0.504&0.504\\
&f1+f4+f5&0.344&0.498&0.498\\
&f2+f4+f5&0.358&0.512&0.512\\
&f3+f4+f5&0.388&0.54&0.54\\

\hline
  DL\_LSTM & - & 0.638 & 0.744 & 0.739 \\
  \hline
  DL\_GRU & - & 0.634 & 0.753 & 0.748 \\

  \hline
  \end{tabular}
  }
\end{table}


\begin{table}
\centering
\caption{F1-Scores for NY Times Dataset}
\label{table:nytimes}
\scalebox{0.65}{
\begin{tabular}{|c|c|c|c|c|}
\hline
Model & Feature Set & Macro & Micro & Weighted \\
\hline
\multirow{12}{4.5em}{Naive Bayes} & f1 & 0.318 & 0.5 & 0.491 \\
 & f2 & 0.326 & 0.515 & 0.504 \\
& f3 & 0.361 & 0.41 & 0.415 \\
& f1 + f4 & 0.3 & 0.335 & .315\\
& f2 + f4 & 0.311 & 0.354 & 0.355\\
& f3 + f4 & 0.359 & 0.407 & 0.421\\
& f1 + f5 & 0.305 & 0.343 & 0.327\\
& f2 + f5 & 0.347 & 0.389 & 0.391\\
& f3 + f5 & 0.377 & 0.426 & 0.439 \\
& f1 + f4 + f5 & 0.319 & 0.354 & 0.353\\
& f2 + f4 + f5 & 0.332 & 0.37 & 0.377\\
& f3 + f4 + f5 & 0.369 & 0.42 & 0.438\\
\hline
\multirow{12}{4.5em}{Decision Tree} & f1 & 0.305 & 0.59 & 0.53 \\
 & f2 & 0.248 & 0.582 & 0.504 \\
 & f3 & 0.295 & 0.477 & 0.413 \\
& f1 + f4 & 0.319 & 0.491 & 0.447 \\
& f2 + f4 & 0.349 & 0.492 & 0.467 \\
 & f3 + f4 & 0.339 & 0.48 & 0.456 \\
 & f1 + f5 & 0.291 & 0.477 & 0.409\\
 & f2 + f5 & 0.357 & 0.524 & 0.481  \\
& f3 + f5 & 0.331 & 0.499 & 0.452 \\
& f1 + f4 + f5 & 0.345 & 0.509 & 0.473 \\
& f2 + f4 + f5 & 0.333 & 0.501 & 0.454 \\
 & f3 + f4 + f5 & 0.333 & 0.496 & 0.456 \\

\hline
\multirow{12}{4.5em}{Random Forest} & f1 & 0.152 & 0.576 & 0.425 \\
& f2 & 0.146 & 0.574 & 0.42 \\
& f3 & 0.219 & 0.453 & 0.339 \\
& f1 + f4 & 0.171 & 0.429 & 0.293 \\
& f2 + f4 & 0.202 & 0.445 & 0.324 \\
& f3 + f4 & 0.201 & 0.444 & 0.321 \\
& f1 + f5 & 0.18 & 0.436 & 0.303 \\
& f2 + f5 & 0.195 & 0.444 & 0.317 \\
& f3 + f5 & 0.206 & 0.446 & 0.327\\
& f1 + f4 + f5 & 0.168 & 0.43 & 0.29\\
& f2 + f4 + f5 & 0.187 & 0.445 & 0.31\\
& f3 + f4 + f5 & 0.199 & 0.447 & 0.321\\
\hline
\multirow{12}{4.5em}{Nearest Neighbors} & f1 & 0.324 & 0.583 & 0.534 \\
 & f2 & 0.279 & 0.567 & 0.514 \\
 & f2 & 0.433 & 0.577 & 0.560 \\
 & f1 + f4 & 0.45 & 0.611 & 0.591 \\
 & f2 + f4 & 0.449 & 0.613 & 0.592 \\
 & f3 + f4 & 0.473 & 0.63 & 0.613 \\
 & f1 + f5 & 0.43 & 0.586 & 0.564 \\
 & f2 + f5 & 0.408 & 0.569 & 0.546\\
 & f3 + f5 & 0.446 & 0.597 & 0.579\\
 & f1 + f4 + f5 & 0.457 & 0.616 & 0.596 \\
 & f2 + f4 + f5 & 0.458 & 0.617 & 0.597 \\
 & f3 + f4 + f5 & 0.478 & 0.635 & 0.619 \\
\hline
% Linear SVM & f1 & 0.116 & 0.411 & 0.239 \\
% Linear SVM & f2 & 0.116 & 0.411 & 0.239 \\
% Linear SVM & f3 & 0.116 & 0.411 & 0.239 \\
% Linear SVM & f1 + f5 & 0.116 & 0.411 & 0.239 \\
% Linear SVM & f2 + f5 & 0.116 & 0.411 & 0.239 \\
% \hline
\multirow{12}{4.5em}{RBF SVM} & f1 & 0.252 & 0.6 & 0.487 \\
 & f2 & 0.216 & 0.601 & 0.491 \\
 & f3 & 0.441 & 0.607 & 0.580 \\
 & f1 + f4 & 0.431 & 0.603 & 0.567 \\
 & f2 + f4 & 0.45 & 0.62 & 0.591 \\
 & f3 + f4 & 0.467 & 0.636 & 0.608\\
 & f1 + f5 & 0.437 & 0.604 & 0.571\\
 & f2 + f5 & 0.418 & 0.586 & 0.556\\
 & f3 + f5 & 0.449 & 0.613 & 0.586\\
 & f1 + f4 + f5 & 0.436 & 0.607 & 0.571\\
 & f2 + f4 + f5 & 0.447 & 0.618 & 0.587\\
 & f3 + f4 + f5 & 0.461 & 0.63 & 0.599\\
\hline
\multirow{12}{4.5em}{Adaboost} & f1 & 0.287 & 0.551 & 0.5 \\
 & f2 & 0.237 & 0.56 & 0.484 \\
 & f3 & 0.310 & 0.454 & 0.426 \\
 & f1 + f4 & 0.322 & 0.45 & 0.429 \\
 & f2 + f4 & 0.316 & 0.452 & 0.427 \\
 & f3 + f4 & 0.344 & 0.481 & 0.458 \\
 & f1 + f5 & 0.345 & 0.476 & 0.454 \\
 & f2 + f5 & 0.332 & 0.463 & 0.439 \\
 & f3 + f5 & 0.342 & 0.477 & 0.456 \\
 & f1 + f4 + f5 & 0.339  & 0.469 & 0.454 \\
 & f2 + f4 + f5 & 0.34  & 0.474 & 0.453 \\
 & f3 + f4 + f5 & 0.357  & 0.493 & 0.475 \\
\hline
\multirow{12}{4.5em}{Logistic Regression} & f1 & 0.192 & 0.571 & 0.444 \\
 & f2 & 0.168 & 0.574 & 0.441 \\
 & f3 & 0.328 & 0.484 & 0.441 \\
 & f1 + f4 & 0.319 & 0.468 & 0.434 \\
 & f2 + f4 & 0.339 & 0.487 & 0.455 \\
 & f3 + f4 & 0.37 & 0.519 & 0.491 \\
 & f1 + f5 & 0.285 & 0.455 & 0.403 \\
 & f2 + f5 & 0.302 & 0.471 & 0.421 \\
 & f3 + f5 & 0.35 & 0.504 & 0.467 \\
 & f1 + f4 + f5 & 0.345 & 0.498 & 0.465 \\
 & f2 + f4 + f5 & 0.359 & 0.512 & 0.482 \\
 & f3 + f4 + f5 & 0.39 & 0.54 & 0.514 \\
\hline
DL\_LSTM & - & 0.638 & 0.744 & 0.739 \\ 
\hline
DL\_GRU & - & 0.645 & 0.791 & 0.780 \\
\hline
\end{tabular}
}
\end{table}


\begin{table}
  \centering
  \caption{Precision scores for NYT Dataset}
  \label{table:guardian}
  \scalebox{0.65}{
  \begin{tabular}{|c|c|c|c|c|}
  \hline
  Model & Feature Set & Macro & Micro & Weighted \\
  
\hline\multirow{12}{4.5em}{Naive Bayes}&f1&0.341&0.5&0.525\\
&f2&0.342&0.515&0.523\\
&f3&0.339&0.472&0.552\\
&f1+f4&0.32&0.303&0.601\\
&f2+f4&0.318&0.311&0.582\\
&f3+f4&0.328&0.33&0.59\\
&f1+f5&0.329&0.348&0.583\\
&f2+f5&0.339&0.38&0.584\\
&f3+f5&0.344&0.384&0.598\\
&f1+f4+f5&0.319&0.311&0.583\\
&f2+f4+f5&0.323&0.339&0.588\\
&f3+f4+f5&0.339&0.352&0.609\\
\hline\multirow{12}{4.5em}{Decision Tree}&f1&0.366&0.59&0.513\\
&f2&0.314&0.582&0.496\\
&f3&0.36&0.583&0.495\\
&f1+f4&0.337&0.605&0.518\\
&f2+f4&0.269&0.564&0.468\\
&f3+f4&0.335&0.578&0.485\\
&f1+f5&0.263&0.586&0.489\\
&f2+f5&0.28&0.567&0.485\\
&f3+f5&0.351&0.59&0.541\\
&f1+f4+f5&0.369&0.592&0.528\\
&f2+f4+f5&0.328&0.588&0.517\\
&f3+f4+f5&0.326&0.584&0.504\\
\hline\multirow{12}{4.5em}{Random Forest}&f1&0.155&0.576&0.366\\
&f2&0.115&0.574&0.331\\
&f3&0.115&0.574&0.33\\
&f1+f4&0.115&0.573&0.33\\
&f2+f4&0.135&0.574&0.348\\
&f3+f4&0.135&0.575&0.343\\
&f1+f5&0.135&0.576&0.347\\
&f2+f5&0.135&0.575&0.34\\
&f3+f5&0.175&0.576&0.378\\
&f1+f4+f5&0.115&0.574&0.329\\
&f2+f4+f5&0.115&0.573&0.33\\
&f3+f4+f5&0.115&0.573&0.329\\
\hline\multirow{12}{4.5em}{Nearest Neighbors}&f1&0.376&0.583&0.518\\
&f2&0.314&0.567&0.493\\
&f3&0.36&0.589&0.525\\
&f1+f4&0.42&0.604&0.558\\
&f2+f4&0.354&0.571&0.519\\
&f3+f4&0.346&0.569&0.529\\
&f1+f5&0.407&0.578&0.52\\
&f2+f5&0.331&0.577&0.521\\
&f3+f5&0.376&0.589&0.534\\
&f1+f4+f5&0.372&0.612&0.559\\
&f2+f4+f5&0.327&0.575&0.525\\
&f3+f4+f5&0.329&0.571&0.53\\
\hline\multirow{12}{4.5em}{RBF SVM}&f1&0.363&0.6&0.483\\
&f2&0.257&0.601&0.462\\
&f3&0.298&0.599&0.481\\
&f1+f4&0.369&0.617&0.519\\
&f2+f4&0.285&0.599&0.476\\
&f3+f4&0.308&0.603&0.493\\
&f1+f5&0.321&0.601&0.481\\
&f2+f5&0.279&0.607&0.479\\
&f3+f5&0.291&0.605&0.481\\
&f1+f4+f5&0.394&0.619&0.54\\
&f2+f4+f5&0.281&0.602&0.474\\
&f3+f4+f5&0.288&0.594&0.477\\
\hline\multirow{12}{4.5em}{AdaBoost}&f1&0.33&0.551&0.483\\
&f2&0.293&0.56&0.467\\
&f3&0.292&0.455&0.449\\
&f1+f4&0.278&0.538&0.471\\
&f2+f4&0.317&0.561&0.476\\
&f3+f4&0.335&0.524&0.477\\
&f1+f5&0.283&0.529&0.484\\
&f2+f5&0.263&0.509&0.454\\
&f3+f5&0.284&0.535&0.463\\
&f1+f4+f5&0.286&0.535&0.474\\
&f2+f4+f5&0.288&0.543&0.481\\
&f3+f4+f5&0.293&0.546&0.472\\
\hline\multirow{12}{4.5em}{Logistic Regression}&f1&0.213&0.571&0.399\\
&f2&0.178&0.574&0.39\\
&f3&0.229&0.593&0.439\\
&f1+f4&0.305&0.59&0.468\\
&f2+f4&0.226&0.586&0.435\\
&f3+f4&0.32&0.606&0.499\\
&f1+f5&0.233&0.575&0.413\\
&f2+f5&0.236&0.583&0.432\\
&f3+f5&0.211&0.587&0.426\\
&f1+f4+f5&0.341&0.6&0.501\\
&f2+f4+f5&0.313&0.598&0.492\\
&f3+f4+f5&0.335&0.601&0.507\\

\hline
  DL\_LSTM & - & 0.638 & 0.744 & 0.739 \\
  \hline
  DL\_GRU & - & 0.634 & 0.753 & 0.748 \\
  \hline
  \end{tabular}
  }
\end{table}


\begin{table}
  \centering
  \caption{Recall scores for NYT Dataset}
  \label{table:guardian}
  \scalebox{0.65}{
  \begin{tabular}{|c|c|c|c|c|}
  \hline
  Model & Feature Set & Macro & Micro & Weighted \\
  
\hline\multirow{12}{4.5em}{Naive Bayes}&f1&0.367&0.5&0.5\\
&f2&0.368&0.515&0.515\\
&f3&0.401&0.472&0.472\\
&f1+f4&0.375&0.303&0.303\\
&f2+f4&0.386&0.311&0.311\\
&f3+f4&0.426&0.33&0.33\\
&f1+f5&0.38&0.348&0.348\\
&f2+f5&0.399&0.38&0.38\\
&f3+f5&0.414&0.384&0.384\\
&f1+f4+f5&0.356&0.311&0.311\\
&f2+f4+f5&0.388&0.339&0.339\\
&f3+f4+f5&0.409&0.352&0.352\\
\hline\multirow{12}{4.5em}{Decision Tree}&f1&0.306&0.59&0.59\\
&f2&0.258&0.582&0.582\\
&f3&0.294&0.583&0.583\\
&f1+f4&0.306&0.605&0.605\\
&f2+f4&0.258&0.564&0.564\\
&f3+f4&0.289&0.578&0.578\\
&f1+f5&0.278&0.586&0.586\\
&f2+f5&0.269&0.567&0.567\\
&f3+f5&0.312&0.59&0.59\\
&f1+f4+f5&0.312&0.592&0.592\\
&f2+f4+f5&0.307&0.588&0.588\\
&f3+f4+f5&0.297&0.584&0.584\\
\hline\multirow{12}{4.5em}{Random Forest}&f1&0.203&0.576&0.576\\
&f2&0.2&0.574&0.574\\
&f3&0.2&0.574&0.574\\
&f1+f4&0.2&0.573&0.573\\
&f2+f4&0.201&0.574&0.574\\
&f3+f4&0.202&0.575&0.575\\
&f1+f5&0.202&0.576&0.576\\
&f2+f5&0.202&0.575&0.575\\
&f3+f5&0.204&0.576&0.576\\
&f1+f4+f5&0.2&0.574&0.574\\
&f2+f4+f5&0.2&0.573&0.573\\
&f3+f4+f5&0.2&0.573&0.573\\
\hline\multirow{12}{4.5em}{Nearest Neighbors}&f1&0.317&0.583&0.583\\
&f2&0.278&0.567&0.567\\
&f3&0.32&0.589&0.589\\
&f1+f4&0.346&0.604&0.604\\
&f2+f4&0.322&0.571&0.571\\
&f3+f4&0.32&0.569&0.569\\
&f1+f5&0.315&0.578&0.578\\
&f2+f5&0.29&0.577&0.577\\
&f3+f5&0.319&0.589&0.589\\
&f1+f4+f5&0.348&0.612&0.612\\
&f2+f4+f5&0.3&0.575&0.575\\
&f3+f4+f5&0.318&0.571&0.571\\
\hline\multirow{12}{4.5em}{RBF SVM}&f1&0.266&0.6&0.6\\
&f2&0.24&0.601&0.601\\
&f3&0.246&0.599&0.599\\
&f1+f4&0.272&0.617&0.617\\
&f2+f4&0.237&0.599&0.599\\
&f3+f4&0.253&0.603&0.603\\
&f1+f5&0.251&0.601&0.601\\
&f2+f5&0.247&0.607&0.607\\
&f3+f5&0.252&0.605&0.605\\
&f1+f4+f5&0.273&0.619&0.619\\
&f2+f4+f5&0.241&0.602&0.602\\
&f3+f4+f5&0.24&0.594&0.594\\
\hline\multirow{12}{4.5em}{AdaBoost}&f1&0.285&0.551&0.551\\
&f2&0.244&0.56&0.56\\
&f3&0.253&0.455&0.455\\
&f1+f4&0.271&0.538&0.538\\
&f2+f4&0.27&0.561&0.561\\
&f3+f4&0.272&0.524&0.524\\
&f1+f5&0.276&0.529&0.529\\
&f2+f5&0.267&0.509&0.509\\
&f3+f5&0.261&0.535&0.535\\
&f1+f4+f5&0.275&0.535&0.535\\
&f2+f4+f5&0.266&0.543&0.543\\
&f3+f4+f5&0.261&0.546&0.546\\
\hline\multirow{12}{4.5em}{Logistic Regression}&f1&0.226&0.571&0.571\\
&f2&0.209&0.574&0.574\\
&f3&0.232&0.593&0.593\\
&f1+f4&0.258&0.59&0.59\\
&f2+f4&0.234&0.586&0.586\\
&f3+f4&0.257&0.606&0.606\\
&f1+f5&0.226&0.575&0.575\\
&f2+f5&0.216&0.583&0.583\\
&f3+f5&0.229&0.587&0.587\\
&f1+f4+f5&0.263&0.6&0.6\\
&f2+f4+f5&0.25&0.598&0.598\\
&f3+f4+f5&0.253&0.601&0.601\\

\hline
  DL\_LSTM & - & 0.638 & 0.744 & 0.739 \\
  \hline
  DL\_GRU & - & 0.634 & 0.753 & 0.748 \\
  \hline
  \end{tabular}
  }
\end{table}
\fi
